Acting upon Imagination: when to trust imagined trajectories in model based reinforcement learning

Model-based reinforcement learning (MBRL) aims to learn model(s) of the environment dynamics that can predict the outcome of its actions. Forward application of the model yields so called imagined trajectories (sequences of action, predicted state-reward) used to optimize the set of candidate actions that maximize expected reward. The outcome, an ideal imagined trajectory or plan, is imperfect and typically MBRL relies on model predictive control (MPC) to overcome this by continuously re-planning from scratch, incurring thus major computational cost and increasing complexity in tasks with longer receding horizon. We propose uncertainty estimation methods for online evaluation of imagined trajectories to assess whether further planned actions can be trusted to deliver acceptable reward. These methods include comparing the error after performing the last action with the standard expected error and using model uncertainty to assess the deviation from expected outcomes. Additionally, we introduce methods that exploit the forward propagation of the dynamics model to evaluate if the remainder of the plan aligns with expected results and assess the remainder of the plan in terms of the expected reward. Our experiments demonstrate the effectiveness of the proposed uncertainty estimation methods by applying them to avoid unnecessary trajectory replanning in a shooting MBRL setting. Results highlight significant reduction on computational costs without sacrificing performance.

==> sections/aui.tex <==
\section{Part II: Acting Upon Imagination}

Based on the discussion and data exploration in the previous section, we will propose two methods on how to avoid recalculating the horizon for few steps and save computation.

%%% Theory
Starting from a state st, one run of the MPPI yields an imagined trajectory comprising a succession of expected states, such that each state \(<s_t, a_t, \hat{s}_{t+1}, \sigma_s_{t+1}, \hat{r}_t>, s_{t},\hat{s}_{t+1}\in S, a_t \in A, \hat{r}_t \in R\). Where $S$ are possible states, $A$ actions, $R$ rewards, and $\sigma_s$ is a confidence bound issued by the dynamics model for the prediction $\hat{s}$.

Executing an action $a_t$ from the imagined trajectory $\tau_s_t$ yields a real-world state $s_{t+1}$ and reward $r_t$, which may differ from the expected state $\hat{s}_{t+1}$ and expected reward $\hat{r}_t$, \(\epsilon_{t+1}= |s_{t+1}-\hat{s}_{t+1}| > 0\).  Building on this information, we propose two methods to determine when it is suitable to continue acting upon imagination, and when to recompute.



\subsection{Confidence Bound (CB) }
Instead of modelling the error of performing an action $a_t$ at state $s_t$ in the real-environment, it is possible to rely on some form of confidence issued by assessing various predicted outcomes of action $a_t$ at state $s_t$, assuming various models\(\hat{f}_1,\ldots,\hat{f}_n\). \ar{adrian rework this, we should describe briefly the types of uncertainty of the model from PETs}
The dynamics model uses an ensemble of neural network models and provides as output the uncertainty of the model $\sigma_s{t+1}$.

So, let us assume that the confidence bound $\sigma_s_{t+1}$ represents the variability in predicted outcomes $\hat{s}_{t+1}$ of an action $a_t$, where the action in question has been deemed appropriate at the given state therefore is in the trajectory. After performing the action, we obtain a real-world state $s_{t+1}$ and compute an error \(\epsilon_{t+1}= |s_{t+1}-\hat{s}_{t+1}|\). The trajectory shall be considered reliable, if the error $\epsilon_{t+1}$ is within the confidence bound $\sigma_s_{t+1}$ of predicted output states obtained from the dynamics model.
Generalizing, if after performing an action at a step ($t+j$,$j >1$ ) the error $\epsilon_{t+j}$ lies within the confidence bound  $\sigma_s_{t+j}$, the trajectory is assumed to be reliable and the agent continues acting upon it. Otherwise, a trajectory is recalculated. The selectivity of the filter is adjusted with a factor of sigma. Which is a hyper parameter to tune.

\textbf{check algorithm}
\begin{algorithm}[tb]
\caption{Confidence Bound Algorithm }
\label{alg:cb_algorithm}
\small
\begin{algorithmic}[1] %[1] enables line numbers
\STATE with dynamics model $\hat{f}(s,a)$\\
\WHILE{task not finished}
\STATE{//Plan T steps ahead:}
\STATE $\textbf{A}^H$ = $controller(s_t)$
\STATE{//Execute first planned action and get state (MPC):}
\STATE $s_{t+1} = env.step(\textbf{A}_{t_{0}}^H)$ 
\STATE{//while the last error fits the confidence bound $sigma$:}
\STATE{//execute the next action and get state:}
\ENDWHILE
\end{algorithmic}
\end{algorithm}

In simple terms, this method assumes that the performance of an action could lead to several possible outcomes, while it trusts the current action. After performing the action, it is observed if the outcome does not deviate from the \emph{bag of expected outcomes} in which case, it is assumed that the trajectory is still reliable.
\textbf{what does this method need as input? is it easier to implement than the firs-step-alike?}

\subsection{Online Dynamics Update}
Until this point, the assumption was that the dynamics model is imperfect and therefore partially reliable, but it does not change. Let us now consider how skipping steps can be used while online updating the dynamics. As the normal case, the environments considered in this paper update the dynamics model online, as described in the algorithm~\ref{alg:pets} (lines AAA--BBBB). 

